CodeRL: Mastering Code Generation through Pretrained Models and Deep Reinforcement Learning

Program synthesis or code generation aims to generate a program that satisfies a problem specification. Recent approaches using large-scale pretrained language models (LMs) have shown promising results, yet they have some critical limitations. In particular, they often follow a standard supervised fine-tuning procedure to train a code generation model only from the pairs of natural-language problem descriptions and ground-truth programs. Such paradigm largely ignores some important but potentially useful signals in the problem specification such as unit tests, which thus often results in poor performance when solving complex unseen coding tasks. To address the limitations, we propose "CodeRL", a new framework for program synthesis tasks through pretrained LMs and deep reinforcement learning (RL). Specifically, during training, we treat the code-generating LM as an actor network, and introduce a critic network that is trained to predict the functional correctness of generated programs and provide dense feedback signals to the actor. During inference, we introduce a new generation procedure with a critical sampling strategy that allows a model to automatically regenerate programs based on feedback from example unit tests and critic scores. For the model backbones, we extended the encoder-decoder architecture of CodeT5 with enhanced learning objectives, larger model sizes, and better pretraining data. Our method not only achieves new SOTA results on the challenging APPS benchmark, but also shows strong zero-shot transfer capability with new SOTA results on the simpler MBPP benchmark.

==> contents/01_abstract.tex <==
Program synthesis or code generation is the task of generating a program given a problem description.
%Recently, we have seen a rising number of deep learning approaches that attempt to address this task in a sequence-to-sequence framework. 
%Recently, several approaches adopted large-scale pretrained language models (LMs) to exploit their contextual representations learned from massive data of codes and natural language.  
While recent large-scale pretrained language models have achieved remarkable results in this domain, 
%these models still perform poorly in complex problems (e.g. interview and competition-level programming). 
we observe two key limitations. 
First, models such as Codex adopt a GPT-style approach in which a Transformer decoder-only architecture is used to process both input and output sequences. %However, in program synthesis, the input sequences contain long and complex problem description in natural language while the output sequences are shorter programs in programming language. 
Secondly, all current models are trained using a conventional next-token prediction objective with perfect program solutions. 
However, during test time, these models generate tokens conditioned on their previously sampled tokens and the resulting sequences are evaluated by their functional correctness against unit tests corresponding to the given problem. 
%Secondly, these models are shown only with perfect solutions and not exposed to imperfect codes. 
%The current discrepancy between training and test time may lead to sub-optimal models, resulting in poor performance in challenging unseen programming tasks during test time. 
To address the first issue, we propose to adopt the encoder-decoder architecture CodeT5 to process the input and output sequences separately. 
We pretrain the models with next-token prediction objective on massive public data.
For the second limitation, we enhance the finetuning process with a deep reinforcement learning (RL) approach.
%Specifically, we obtain synthetic training samples of both correct and incorrect codes.
In order to provide dense feedback signals to the code generating LM (actor network), we introduce a critic network that is trained to predict the functional correctness of synthetic code samples. 
%We introduce a critic network that is trained to evaluate functional correctness of synthetic samples by predicting their unit testing results. 
%We use the token-level hidden states from the critic model to estimate %relative returns
%the value of output tokens of synthetic samples and train an actor network. 
%We use the trained critic network to measure the expected values of output tokens and optimize language models as an actor network. 
%This strategy allows us to optimize models by exploiting training samples that are valuated by their expected computation correctness. 
We show that our approach can achieve SOTA performance on the APPS benchmark, with consistent performance gains on competition-level programming problems. 
%We achieved SOTA on the APPS benchmark with 2.2\% pass@1, 3.1\% pass@5, and more than 12\% pass@k with large-scale sampling generation on a 770M-CodeT5.

\iffalse
Program synthesis or code generation is the task of generating a program given a problem description. While recent large-scale pretrained language models have achieved remarkable results in this domain, we observe two key limitations. First, models such as Codex adopt a GPT-style approach in which a Transformer decoder-only architecture is used to process both input and output sequences. Secondly, all current models are trained using a conventional next-token prediction objective with perfect program solutions. However, during test time, these models generate tokens conditioned on their previously sampled tokens and the resulting sequences are evaluated by their functional correctness against unit tests corresponding to the given problem. To address the first issue, we propose to adopt the encoder-decoder architecture CodeT5 to process the input and output sequences separately. 
We pretrain the models with next-token prediction objective on massive public data.
For the second limitation, we enhance the finetuning process with a deep reinforcement learning (RL) approach. In order to provide dense feedback signals to the code generating LM (actor network), we introduce a critic network which is trained to predict the functional correctness of synthetic code samples. We show that our approach can achieve SOTA performance on the APPS benchmark, with consistent performance gains on competition-level programming problems. 
\fi

==> contents/01_abstract_v1.tex <==
Program synthesis is the task of generating a program given a problem description.
%Recently, we have seen a rising number of deep learning approaches that attempt to address this task in a sequence-to-sequence framework. 
%Recently, several approaches adopted large-scale pretrained language models (LMs) to exploit their contextual representations learned from massive data of codes and natural language.  
While recent large-scale pretrained language models have achieve remarkable results in this domain, 
%these models still perform poorly in complex problems (e.g. interview and competition-level programming). 
we observe two key limitations. 
First, models such as Codex adopt a GPT-style approach in which a Transformer decoder-only architecture is used to process both input and output sequences. %However, in program synthesis, the input sequences contain long and complex problem description in natural language while the output sequences are shorter programs in programming language. 
Secondly, all current models are trained using a conventional next-token prediction objective with perfect program solutions. 
However, during test time, these models generate tokens conditioned on their previously sampled tokens and the resulting sequences are tested by their computation correctness against some unit tests. 
%Secondly, these models are shown only with perfect solutions and not exposed to imperfect codes. 
The current discrepancy between training and test time may lead to sub-optimal models, resulting in poor performance in challenging unseen programming tasks during test time. 
To address these issues, we propose to adopt the encoder-decoder architecture CodeT5 to process the input and output sequences separately. 
We pretrain the models with next-token prediction objective on massive public data.
Secondly, we enhance the finetuning process with a deep reinforcement learning (RL) approach.
%Specifically, we obtain synthetic training samples of both correct and incorrect codes.
We introduce a critic network that is trained to evaluate functional correctness of synthetic samples by predicting their unit testing results. 
%We use the token-level hidden states from the critic model to estimate %relative returns
%the value of output tokens of synthetic samples and train an actor network. 
We use the trained critic network to measure the expected values of output tokens and optimize language models as an actor network. 
%This strategy allows us to optimize models by exploiting training samples that are valuated by their expected computation correctness. 
We show that our models can achieve promising performance on the APPS benchmark, with consistent performance gains on competition-level programming problems. 
%We achieved SOTA on the APPS benchmark with 2.2\% pass@1, 3.1\% pass@5, and more than 12\% pass@k with large-scale sampling generation on a 770M-CodeT5.


==> contents/02_introduction.tex <==
\section{Introduction}
Considering program synthesis as a sequence-to-sequence task, pretrained language models (LMs) \citep{hendrycksapps2021, chen2021evaluating, austin2021program} can be adapted to receive input sequence as problem statement in natural language and generate a sequence of codes as the output program (See Figure \ref{fig:example_program} for an example).
%(See Figure \ref{fig:sample} for an example). 
While these models achieve promising results, especially in basic programming tasks \citep{chen2021evaluating, austin2021program}, we observe that they still fail to generate codes to solve complex problems \citep{hendrycksapps2021, li2022competition}.

There are two main limitations. 
First, current models are trained using a conventional next-token prediction objective which maximizes the next ground-truth token. 
As noted by prior work in NLP domains \cite{bengio2015scheduled, DBLP:journals/corr/RanzatoCAZ15}, training models only with next-token prediction objective in a "teacher-forcing" manner often leads to a accumulating errors during test time when tokens are generated by conditioning on previously sampled tokens. 
Moreover, specifically in the program synthesis domain, this optimization strategy neglects the important signals from unit tests
%(See Figure \ref{fig:sample} for an example) 
which during test time, directly determine the functional correctness of output programs. 

%Moreover, these models are affected by exposure bias \citep{DBLP:journals/corr/RanzatoCAZ15} as they are trained with only perfect ground-truth reference programs without any exposure to imperfect codes. 
%Unlike these models, human programmers are exposed to variants of codes and learn to compare them (by complexities, potential errors, etc.) before writing their own version of codes. 
%The current model training strategy may prevent models from exploring feature space necessary for solving complex programming tasks. 
\begin{figure}[t]
	\centering
	\resizebox{1.0\textwidth}{!} {
	\includegraphics{figures/example_program.pdf}
	}
	\caption{An example program synthesis task: 
	The input is a problem description in natural language and the output is a program in programming language. 
	To evaluate, the program is passed to unit tests and the test outputs are checked against ground-truth outputs.}
	\label{fig:example_program}
\end{figure}
Secondly, existing state-of-the-art program synthesis models such as Codex \citep{chen2021evaluating} adopt a GPT-style approach in which a Transformer decoder-only architecture is used to process both input and output sequences. 
However, in program synthesis tasks, the input and output sequences are fundamentally different in two aspects: 
(1) Language: the input sequences are problem descriptions in natural language while the output sequences are codes in programming language.
(2) Length: the problem descriptions are often long and complex, sometimes including background stories and even embedded images. 
Conversely, the output sequences are concise pieces of codes and interpreting these codes strictly depends on specific syntax of programming languages.

To address the above issues, we propose to extend CodeT5 \citep{codet5} for program synthesis tasks and alter model optimization with reinforcement learning (RL) \citep{sutton2018reinforcement} (See Figure \ref{fig:rl_approach} for an overview). 
The encoder-decoder architecture of CodeT5 allows us to segregate the processing networks of input and output sequences, creating an architectural bias that is appropriate for program synthesis tasks. Unlike the decoder only architecture, encoder-decoder models allow a bidirectional representation where tokens at the beginning of the input can attend to the tokens at the end. We pretrain CodeT5 models with next-token prediction objective on massive public data.
%relased by HuggingFace \citep{lhoest-etal-2021-datasets}. 
We then finetune these models for program synthesis tasks with an actor-critic framework \citep{sutton1984temporal, konda1999actor, sutton1999policy}.
Specifically, we treat the pretrained LM as an actor network and sample sequences from the actor, including both correct and incorrect programs.
These samples are passed to a critic model which is trained as an error predictor to assess the functional correctness of these samples.
We use the token-level hidden states extracted from the learned critic model to estimate the values of output tokens of these synthetic samples. 
We then finetune the actor with these synthetic samples weighted by their critic scores. 
%This finetuning framework allows us to optimize models by exploiting training samples that are valuated by their expected computation correctness. 

We denote the overall framework as ``CodeRL'' and show that models finetuned with CodeRL can achieve SOTA performance on the APPS benchmark \citep{hendrycksapps2021}.
Specifically, our models can obtain 2.2\% pass@1, 3.1\% pass@5, and more than 17\% pass@1000. 
%We experiment with a sampling approach by filtering samples and selecting sub-sequences as seeds to the LMs to refine programs.
%This sampling method bring the performance up to 20\% pass@1000.
Since our RL method is model-agnostic, we apply it to various large-scale models and achieve consistent performance gains.  
We release a CodeT5-large (770M) which demonstrates superior performance against many GPT-style models of much larger sizes.

%We also applied our RL approaches with other GPT-style models and obtained consistent performance gains. 


==> contents/02_introduction_v0.tex <==
\section{Introduction}
\iffalse
\begin{figure}[htbp]
	\centering
	\resizebox{1.0\textwidth}{!} {
	\includegraphics{figures/apps.pdf}
	}
	\caption{(Sample Figure from APPS, to be replaced by our own figure) An example of program synthesis task}
	\label{fig:sample}
\end{figure}
\fi
Considering program synthesis as a sequence-to-sequence task, pretrained language models (LMs) \citep{hendrycksapps2021, chen2021evaluating, austin2021program} can be adapted to receive input sequence as problem statement in natural language and generate a sequence of codes as the output program (See Figure \ref{fig:example_program} for an example).
%(See Figure \ref{fig:sample} for an example). 
While these models achieve promising results, especially in basic programming tasks \citep{chen2021evaluating, austin2021program}, we observe that they still fail to generate codes to solve complex problems \citep{hendrycksapps2021, li2022competition}.

There are two main limitations. 
First, current models are trained using a conventional next-token prediction objective which maximizes the next ground-truth token. 
However, this objective does not integrate signals from unit tests
%(See Figure \ref{fig:sample} for an example) 
which during test time, directly determine the correctness of output programs. 
As noted by prior work in NLP domains \cite{bengio2015scheduled, DBLP:journals/corr/RanzatoCAZ15}, training models only with next-token prediction objective in a "teacher-forcing" manner often leads to a mismatch between training and test time.
Specifically in program synthesis task, this strategy neglects the important signals from unit tests and lead to sub-optimal models. 
Moreover, these models are affected by exposure bias \citep{DBLP:journals/corr/RanzatoCAZ15} as they are trained with only perfect ground-truth reference programs without any exposure to imperfect codes. 
Unlike these models, human programmers are exposed to variants of codes and learn to compare them (by complexities, potential errors, etc.) before writing their own version of codes. 
%The current model training strategy may prevent models from exploring feature space necessary for solving complex programming tasks. 
\begin{figure}[t]
	\centering
	\resizebox{1.0\textwidth}{!} {
	\includegraphics{figures/example_program.pdf}
	}
	\caption{An example program synthesis task}
	\label{fig:example_program}
\end{figure}

Secondly, existing SOTA program synthesis models such as Codex \citep{chen2021evaluating} adopts a GPT-style approach in which a Transformer decoder-only architecture is used to process both input and output sequences. 
However, in program synthesis tasks \citep{hendrycksapps2021, austin2021program}, the input and output sequences are fundamentally different in two dimensions: 
(1) languages: the input sequences are problem descriptions in natural language while the output sequences are codes in programming language.
(2) lengths: the problem descriptions are often long and complex, sometimes including background stories and even embedded images. 
Conversely, the output sequences are concise pieces of codes and interpreting these codes exclusively depends on specific syntax of programming languages such as Java and Python. 

To address the above issues, we propose to extend CodeT5 \citep{codet5} and integrates the models with RL finetuning techniques \citep{sutton2018reinforcement} (See Figure \ref{fig:rl_approach} for an overview). 
The encoder-decoder architecture CodeT5 allows us to segregate the processing networks of input and output sequences, creating an architectural bias that is appropriate for program synthesis tasks. 
We pretrain the models with next-token prediction objective on massive public data.
%relased by HuggingFace \citep{lhoest-etal-2021-datasets}. 
We finetune the models for program synthesis tasks with an actor-critic framework \citep{sutton1984temporal, konda1999actor, sutton1999policy}.
Specifically, we treat the pretrained LM as an actor network and sample sequences from the actor, including both correct and incorrect programs.
These samples are passed to a critic model which is learned as an error predictor to assess the computation correctness of these samples.
We use the token-level hidden states extracted from the learned critic model to estimate the values of output tokens of these synthetic samples. 
We then finetune the actor with these synthetic samples weighted by their critic-based token-level values. 
%This finetuning framework allows us to optimize models by exploiting training samples that are valuated by their expected computation correctness. 

We show that our models can achieve SOTA performance on the APPS benchmark \citep{hendrycksapps2021}.
Specifically, our models can obtain 2.2\% pass@1, 3.1\% pass@5, and more than 17\% pass@1000. 
We experimented with a sampling approach by filtering samples and selecting sub-sequences as seeds to the LMs to refine programs.
This sampling method bring the performance up to 20\% pass@1000.
Since our RL method is model-agnostic, we applied on various large-scale models and achieve consistent performance gains.  
%We release a CodeT5-large (770M) which demonstrates superior performance against many GPT-style models of much larger sizes. 
%We also applied our RL approaches with other GPT-style models and obtained consistent performance gains. 


==> tables/codet5_ablation.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation results of CodeT5 model variants with different sizes, pretraining data and objectives}
% \begin{tabular}{ccccccc}
% \hline 
% Size & \begin{tabular}[c]{@{}c@{}}Pretraining\\ Data\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretraining \\ Objective\end{tabular} & Introductory & Interview & Competition & All  \\ \hline 
% 60M  & CSN                                                        & MSP                                                               & 1.60         & 0.60      & 0.00        & 0.68 \\
% 220M & CSN                                                        & MSP                                                               & 2.00         & 0.80      & 0.20        & 0.92 \\
% 770M & CSN                                                        & MSP                                                               & 3.70         & 0.80      & 0.00        & 1.22 \\
% 770M & +GCPY                                                     & MSP                                                               & 3.80         & 0.93      & 0.10        & 1.34 \\
% 770M & +GCPY                                                     & +NTP                                                             & 6.60         & 1.03      & 0.30        & 2.00 \\
% \hline 
% \end{tabular}
\begin{tabular}{cccccccc}
\hline 
Size & \begin{tabular}[c]{@{}c@{}}Pretraining\\ Data\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretraining \\ Objective\end{tabular}  & Attempts & Introductory & Interview & Competition & All  \\ \hline 
60M  & CSN                                                        & MSP     & 1                                                          & 1.40         & 0.67      & 0.00        & 0.68 \\
220M & CSN                                                        & MSP    & 1                                                             & 2.50         & 0.73      & 0.00        & 0.94 \\
770M & CSN                                                        & MSP         & 1                                                        & 3.60         & 0.90         & 0.20        & 1.30 \\
770M & +GCPY                                                     & MSP        & 1                                                         & 4.30         & 1.10      & 0.20        & 1.56 \\
770M & +GCPY                                                     & +NTP      & 1                                                         & 6.60         & 1.03      & 0.30        & 2.00 \\
\hline 
60M  & CSN                                                        & MSP     & 5                                                          &  2.60       &  0.87   &  0.10      & 1.06 \\
220M & CSN                                                        & MSP    & 5                                                            & 3.30         & 1.10      & 0.10        & 1.34 \\
770M & CSN                                                        & MSP         & 5                                                        & 4.30            & 1.37       & 0.20        & 1.72 \\
770M & +GCPY                                                     & MSP        & 5                                                         & 5.60         & 1.47      & 0.30        & 2.06 \\
770M & +GCPY                                                     & +NTP      & 5                                                         & 8.80         & 1.67      & 0.70        & 2.90 \\
\hline 
\end{tabular}
\end{table}


==> tables/codet5_ablation_by_loss.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation results of CodeT5 models trained with different combinations of loss functions:} 
%\resizebox{1.0\textwidth}{!} {
\begin{tabular}{llccccc}
\hline
CE loss & RL loss & Attempts & Introductory & Interview & Competition & All  \\ \hline 
pretrained                  &   -      & 1        & 6.60         & 1.03      & 0.30        & 2.00 \\
\checkmark                           &    -     & 1        & 4.60         & 0.93      & 0.10        & 1.50 \\
\checkmark (+$W^s$)             &   -      & 1        & 5.10         & 1.10      & 0.40        & 1.76 \\
         -                   & \checkmark       & 1        & 5.00         & 0.90      & 0.50        & 1.64 \\
%\checkmark (shared)                          & \checkmark (shared)     & 1        & 5.50	& 1.33 &	0.30	& 1.96 \\
\checkmark                           & \checkmark       & 1        & 6.20         & 1.50      & 0.30        & 2.20 \\
\hline
pretrained                  &  -       & 5        & 8.80         & 1.67      & 0.70        & 2.90 \\
\checkmark                           &   -      & 5        & 7.00         & 1.37      & 0.20        & 2.26 \\
\checkmark (+$W^s$)             &   -      & 5        & 8.30         & 1.43      & 0.70        & 2.66 \\
         -                   & \checkmark       & 5        & 7.60         & 1.53      & 0.60        & 2.56 \\
%\checkmark (shared)                          & \checkmark (shared)     & 5        & 7.50	&1.90&	0.50&	2.74\\
\checkmark                           & \checkmark       & 5        & 9.39         & 1.90      & 0.42        & 3.10\\

\hline
\end{tabular}
%}
\end{table}

==> tables/codet5_ablation_by_loss_v2.tex <==




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\small
\caption{Ablation results of models trained with different combinations of loss functions:} 
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{cccccccccccccccccc}
\multirow{3}{*}{$\mathcal{L}_{ce}$} & \multirow{3}{*}{$\mathcal{L}_{rl}$} & \multicolumn{8}{c}{GPT-Neo}                               & \multicolumn{8}{c}{CodeT5-770M}                           \\
                         &                          & \multicolumn{4}{c}{k=1}     & \multicolumn{4}{c}{k=5}     & \multicolumn{4}{c}{k=1}     & \multicolumn{4}{c}{k=5}     \\
                         &                          & Intro & Inter & Comp & All  & Intro & Inter & Comp & All  & Intro & Inter & Comp & All  & Intro & Inter & Comp & All  \\
-                        & -                        & 3.90  & 0.57  & 0.00 & 1.12 & 5.50  & 0.80  & 0.00 & 1.58 & 6.60  & 1.03  & 0.30 & 2.00 & 8.80  & 1.67  & 0.70 & 2.90 \\
\checkmark                        & -                        & 2.70  & 0.90  & 0.10 & 1.10 & 5.00  & 1.43  & 0.30 & 1.92 & 4.60  & 0.93  & 0.10 & 1.50 & 7.00  & 1.37  & 0.20 & 2.26 \\
\checkmark($+{W}^s$)                   & -                        & 2.90  & 0.80  & 0.30 & 1.12 & 5.20  & 1.57  & 0.40 & 2.06 & 5.10  & 1.10  & 0.40 & 1.76 & 8.30  & 1.43  & 0.70 & 2.66 \\
-                        & \checkmark                        & 3.30  & 0.80  & 0.20 & 1.18 & 5.30  & 1.57  & 0.20 & 2.04 & 5.00  & 0.90  & 0.50 & 1.64 & 7.60  & 1.53  & 0.60 & 2.56 \\
\checkmark                        & \checkmark                        & 4.70  & 0.73  & 0.30 & 1.44 & 6.58  & 1.54  & 0.18 & 2.28 & 6.20  & 1.50  & 0.30 & 2.20 & 9.39  & 1.90  & 0.42 & 3.10
\end{tabular}
}
\end{table}





==> tables/codet5_ablation_by_return.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation results of CodeT5 models trained with RL with different frameworks to estimate returns: by return level, return type, and return estimator.}
\begin{tabular}{cccccccc}
\hline
\begin{tabular}[c]{@{}c@{}}Return \\ level\end{tabular} & \begin{tabular}[c]{@{}c@{}}Return \\ type\end{tabular} & \begin{tabular}[c]{@{}c@{}}Return \\ model\end{tabular} & Attempts & Introductory & Interview & Competition & All  \\\hline
Sequence     & Relative    & None        & 1            & 4.60         & 1.10      & 0.20        & 1.62 \\
Token        & Absolute    & Critic        & 1            & 4.00         & 0.87      & 0.20        & 1.36 \\
Token        & Relative    & Distance      & 1            & 4.90         & 1.03      & 0.20        & 1.64 \\
Token        & Relative    & Critic        & 1            & 6.20         & 1.50      & 0.30        & 2.20 \\\hline
Sequence     & Relative    & None        & 5            & 7.10         & 1.57      & 0.40        & 2.44 \\
Token        & Absolute    & Critic        & 5            & 5.60         & 1.30      & 0.20        & 1.94 \\
Token        & Relative    & Distance      & 5            & 7.80         & 1.60      & 0.30        & 2.58 \\
Token        & Relative    & Critic        & 5            & 9.39         & 1.90      & 0.42        & 3.10 \\
\hline
\end{tabular}
\end{table}

==> tables/codet5_ablation_mbpp.tex <==
\begin{table}[t]
\centering
\small
\caption{Ablation results of CodeT5 model variants with different sizes, pretraining data and objectives on MBPP. CodeT5 (APPS) is finetuned on APPS and evaluated on MBPP in a zero-shot setting. Results of GPT models are obtained from the original authors.}\label{tab:mbpp}
\begin{tabular}{cc|cc|ccc}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Size} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pretraining\\ Data\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pretraining\\ Objective\end{tabular}} & \multirow{2}{*}{\emph{pass@10} }   & \multirow{2}{*}{\emph{pass@80}}  & \multirow{2}{*}{\emph{pass@1000}}     \\
&     &         &         &        &  & \\
\hline
\multicolumn{7}{c}{\cellcolor[HTML]{EFEFEF}Pretrained GPT} \\
\hline
GPT & 224M & Web Doc   & LM     & - & 7.2 & -\\ 
GPT & 422M & Web Doc   & LM     & - & 12.6 & -\\ 
GPT & 1B & Web Doc   & LM     & - & 22.4 & -\\       
GPT & 4B & Web Doc   & LM     & - & 33.0 & -\\   
GPT & 8B & Web Doc   & LM     & - & 40.6 & -\\   
GPT & 68B & Web Doc   & LM     & - & 53.6 & -\\   
GPT & 137B & Web Doc   & LM     & - & 61.4 & -\\   
\hline
\multicolumn{7}{c}{\cellcolor[HTML]{EFEFEF}Pretrained CodeT5} \\
\hline
  
CodeT5 & 60M                   & CSN                                                                              & MSP           & 8.6 & 15.4 & 22.8 \\
CodeT5 &220M                  & CSN                                                                              & MSP         & 11.0 & 16.0 & 20.2 \\
CodeT5 &770M                  & CSN                                                                              & MSP         & 15.2 & 20.0 & 25.6 \\
CodeT5 &770M                  & +GCPY                                                                            & MSP         & 18.2 & 27.2 & 35.2         \\
CodeT5 &770M                  & +GCPY                                                                            & +NTP        & 26.8 & 46.8 & 44.8\\
CodeT5 (APPS) &770M                  & +GCPY                                                                            & +NTP        & 41.4 & 63.4 & 73.4\\
% \hline
% \multicolumn{7}{c}{\cellcolor[HTML]{EFEFEF}Pretrained CodeT5 + CodeRL} \\
% \hline
% CodeT5 &770M                  & +GCPY                                                                            & +NTP        & - & -& - \\
\hline
\end{tabular}
\end{table}

==> tables/codet5_ablation_v1.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\small
\caption{Ablation results of CodeT5 model variants with different sizes, pretraining data and objectives}
\begin{tabular}{ccc|cccc|cccc}
\hline
\multirow{2}{*}{Size} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pretraining\\ Data\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pretraining\\ Objective\end{tabular}} & \multicolumn{4}{c|}{\emph{pass@1}}     & \multicolumn{4}{c}{\emph{pass@5}}     \\
\cline{4-11}
                      &                                                                                  &                                                                             & Intro & Inter & Comp & All  & Intro & Inter & Comp & All  \\
                      \hline
60M                   & CSN                                                                              & MSP                                                                         & 1.40  & 0.67  & 0.00 & 0.68 & 2.60  & 0.87  & 0.10 & 1.06 \\
220M                  & CSN                                                                              & MSP                                                                         & 2.50  & 0.73  & 0.00 & 0.94 & 3.30  & 1.10  & 0.10 & 1.34 \\
770M                  & CSN                                                                              & MSP                                                                         & 3.60  & 0.90  & 0.20 & 1.30 & 4.30  & 1.37  & 0.20 & 1.72 \\
770M                  & +GCPY                                                                            & MSP                                                                         & 4.30          & \textbf{1.10} & 0.20          & 1.56          & 5.60          & 1.47          & 0.30          & 2.06          \\
770M                  & +GCPY                                                                            & +NTP                                                                        & \textbf{6.60} & 1.03          & \textbf{0.30} & \textbf{2.00} & \textbf{8.80} & \textbf{1.67} & \textbf{0.70} & \textbf{2.90} \\
\hline
\end{tabular}
\end{table}

==> tables/codet5_codexglue_code2code.tex <==
\begin{table}[t]
\centering
\caption{Code-to-Code generation results on CodeXGLUE}
\label{app_tab:codexglue_code2code}

\begin{tabular}{l| cc | c c  | c c | c c}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Java to C\#} & \multicolumn{2}{c|}{C\# to Java}  & \multicolumn{2}{c|}{Refine Small}  & \multicolumn{2}{c}{Refine Medium}\\ 
\cline{2-9}
& BLEU & EM  & BLEU & EM & BLEU & EM & BLEU & EM  \\ 
\hline 
Naive copy & 18.54 & 0.00 & 18.69 & 0.00 & 78.06 & 0.00 & 90.91 & 0.00 \\ 
        Roborta (code) & 77.46 & 56.10 & 71.99 & 57.90 & 77.30 & 15.90 & 90.07 & 4.10 \\ 
        CodeBERT & 79.92 & 59.00 & 72.14 & 58.00 & 77.42 & 16.40 & 91.07 & 5.20 \\ 
        GraphCodeBERT & 80.58 & 59.40 & 72.64 & 58.80 & \textbf{80.02} & 17.30 & \textbf{91.31} & 9.10 \\ 
        PLBART & 83.02 & 64.60 & 78.35 & 65.00 & 77.02 & 19.21 & 88.50 & 8.98 \\ 
        CoTexT & - & - & - & - & 77.79 & 21.03 & 88.40 & 13.11 \\ 
        NSEdit & - & - & - & - & 71.06 & \textbf{24.04} & 85.72 & 13.87 \\ 
        CodeT5-small & 82.98 & 64.10 & 79.10 & 65.60 & 76.23 & 19.06 & 89.20 & 10.92 \\ 
        CodeT5-base & \textbf{84.03} & 65.90 & \textbf{79.87} & 66.90 & 77.43 & 21.61 & 87.64 & 13.96 \\ 
\hline        
        CodeT5-large & 83.56 & \textbf{66.00} & 79.77 & \textbf{67.00} & 77.38 & 21.70 & 89.22 & \textbf{14.76} \\ 
\hline
\end{tabular}
\end{table}

==> tables/codet5_codexglue_code2text.tex <==
\begin{table*} [t]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{12cm}p{7cm}}
\begin{minipage}{0.87\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c c c c c c|c}
\hline
Model & Ruby & JS & Go & Python & Java & PHP & Overall \\
\hline
RoBERTa  & 11.17 & 11.90 & 17.72 & 18.14 & 16.47 & 24.02 & 16.57 \\
CodeBERT & 12.16 & 14.90 & 18.07 & 19.06 & 17.65 & 25.16 & 17.83 \\ 
DOBF & -& -& -  &18.24 & 19.05 & - & - \\
PLBART &  14.11 &  15.56 &  18.91 & 19.30 & 18.45 & 23.58 & 18.32\\
CoTexT & 14.02	 &14.96	 &18.86	 &19.73	 &19.06	 &24.58	 & 18.55 \\
CodeT5-small & 14.87&	15.32&	19.25&	20.04&	19.92&	25.46&	19.14\\
CodeT5-base & 15.24&	16.16&	19.56&	20.01&	20.31&	26.03&	19.55\\
\hline
CodeT5-large &\textbf{15.58}	&\textbf{16.17}	&\textbf{19.69}	&\textbf{20.57}	&\textbf{20.74}&	\textbf{26.49}	&\textbf{19.87} \\
\hline
\end{tabular}
}
\captionsetup{type=table}
\vspace{-0.5em}  
\caption{
BLEU scores and exact match (EM) accuracies for code translation and code refinement tasks.
}
\label{table:code_translation}

\end{minipage}

&
\begin{minipage}{0.58\textwidth}
\resizebox{\textwidth}{!}{

\begin{tabular}{l|ccc}
\hline
Model         & EM    & BLEU  & CodeBLEU \\
\hline
% GPT-2           & 17.35 & 25.37 & 29.69    \\
CodeGPT-2       & 18.25 & 28.69 & 32.71    \\
CodeGPT-adapted & 20.10 & 32.79 & 35.98    \\
PLBART          & 18.75 & 36.69 & 38.52    \\
CoTexT          & 20.10 & 37.40 & 40.14    \\
UniXcoder       & 22.60 & 38.23 & -        \\
CodeT5-small    & 21.55 & 38.13 & 41.39    \\
CodeT5-base     & 22.30 & 40.73 & 43.20    \\
\hline
CodeT5-large    & 22.65 & 42.66 & 45.08   \\
\hline
\end{tabular}
}
\captionsetup{type=table}
% \vspace{-0.5em}  
\caption{Results on the code defect detection  and clone detection  tasks.}
% }
\label{table:classification}

\end{minipage}
\end{tabular}
}
\end{center}
% \vspace{-2em}
\end{table*}



==> tables/codet5_gsm.tex <==
\begin{table}[t] %{rt}{0.4\textwidth}
%\vspace{-0.2in}
\centering
%\small
% (CodeT5$^{\dag}$ is finetuned on APPS)
\caption{GSM8K-Python benchmark results. $^{\dag}$: few-shot learning results}
\label{tab:codet5_gsm}
%\resizebox{0.4\textwidth}{!} {
\begin{tabular}{lc|cc}
\hline
Model & Size & \emph{pass@1} & \emph{pass@100} \\
\hline
OpenAI & 6B & 21.8 & 70.9 \\
PaLM-Coder$^{\dag}$ & 540B & \textbf{50.9} & - \\
GPT$^{\dag}$ & 137B & 7.6 & - \\
Codex Davinci$^{\dag}$  & - & 17.0 & 71.0 \\
GPT-Neo (self-sampling) & 2.7B & 19.5 & 41.4 \\
\hline
CodeT5 & 770M & 26.2 & \textbf{73.8} \\
\hline
\end{tabular}
%}
%\vspace{-0.1in}
\end{table}

==> tables/codet5_mathqa.tex <==
\begin{table}[t] %{rt}{0.4\textwidth}
%\vspace{-0.2in}
\centering
%\small
% (CodeT5$^{\dag}$ is finetuned on APPS)
\caption{MathQA-Python benchmark results. $^{\dag}$: few-shot learning results}
\label{tab:codet5_mathqa}
%\resizebox{0.4\textwidth}{!} {
\begin{tabular}{lc|c}
\hline
Model & Size & \emph{pass@80} \\
\hline
Codex Davinci$^{\dag}$  & - & 42.0 \\
GPT & 8B & 74.7 \\
GPT & 68B & 79.5 \\
GPT & 137B & 81.2 \\
GPT-Neo (self-sampling) & 125M & 84.7 \\
\hline
CodeT5 & 770M & \textbf{87.4} \\
\hline
\end{tabular}
%}
%\vspace{-0.1in}
\end{table}

==> tables/critic_sampling.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
%{r}{0.5\textwidth}
%\vspace{-0.1in}
%\small
\centering
\caption{Ablation results of critic sampling}
\label{tab:critic_sampling}
%\resizebox{0.5\textwidth}{!} {
\begin{tabular}{lccccc}
\hline
\multicolumn{1}{c}{Metric} & Approach   & Intro & Inter & Comp  & All   \\ \hline
\multirow{2}{*}{\emph{pass@200}} & without CS & 26.79 &	8.73 &	7.60 &	12.12 \\
                           & with CS    & 29.10 &	9.67 &	9.50 &	13.52 \\
                           \hline
\multirow{2}{*}{\emph{pass@1000}} & without CS & 35.30 & 13.33 & 13.60 & 17.78 \\
                           & with CS    & 38.10 & 14.33 & 15.70 & 19.36 \\
                           \hline
\multirow{2}{*}{\emph{1@1000}}    & without CS & 16.27 & 6.00  & 4.27  & 7.71  \\
                           & with CS    & 16.52 & 6.16  & 4.15  & 7.83  \\ \hline
%\multirow{2}{*}{\emph{5@1000}}    & without CS & 24.78 & 8.75  & 8.33  & 11.87 \\
%                           & with CS    & 24.49 & 8.58  & 7.82  & 11.61 \\
%                           \hline
\end{tabular}
%}
%\vspace{-0.1in}
\end{table}

==> tables/gptneo_ablation_by_loss.tex <==

\begin{table}[htbp]
\centering
\caption{Ablation results of GPT-Neo models trained with different combinations of loss functions:} 
\begin{tabular}{llccccc}
\hline
CE loss         & RL loss & Attempts & Introductory & Interview & Competition & All  \\ 
\hline
pretrained      &  -       & 1        & 3.90         & 0.57      & 0.00        & 1.12 \\
\checkmark               &  -       & 1        & 2.70         & 0.90      & 0.10        & 1.10 \\
\checkmark (+$Y_{rl}$) &   -      & 1        & 2.90         & 0.80      & 0.30        & 1.12 \\
   -             & \checkmark       & 1        & 3.30         & 0.80      & 0.20        & 1.18 \\
%\checkmark (shared)              & \checkmark (shared)      & 1        & 3.10&	0.77&	0.50&	1.18 \\
\checkmark               & \checkmark       & 1        & 4.70         & 0.73      & 0.30        & 1.44 \\
\hline
pretrained      &   -      & 5        & 5.50         & 0.80      & 0.00        & 1.58 \\
\checkmark               &   -      & 5        & 5.00         & 1.43      & 0.30        & 1.92 \\
\checkmark (+$Y_{rl}$) &  -       & 5        & 5.20         & 1.57      & 0.40        & 2.06 \\
        -        & \checkmark       & 5        & 5.30         & 1.57      & 0.20        & 2.04 \\
%\checkmark (shared)              & \checkmark (shared)      & 5        & 5.10&	1.50&	0.60&	2.04 \\
\checkmark               & \checkmark       & 5        & 6.58         & 1.54      & 0.18        & 2.28 \\ 
\hline
\end{tabular}
\end{table}

==> tables/n_pass_k.tex <==
\begin{table}[htbp]
\centering
\caption{Results of $1@k$ on APPS:}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lccccccc}
\hline
Model     & Size & Filter from & Attempts & Introductory & Interview & Competition & All   \\
\hline
Codex     & 12B  & 1000        & 1        & 22.78        & 2.64      & 3.04        & 6.75  \\
\hline
GPT-J  & 6B   & 100         & 1        &    12.24	& 4.85	& 1.91	& 5.74 \\
GPT-J+RL  & 6B   & 100         & 1        & 13.08        & 4.93      & 2.26        & 6.03  \\
\hdashline
GPT-J  & 6B   & 200         & 1        &    13.40	 & 5.35	 & 2.40	 & 6.37 \\
GPT-J+RL  & 6B   & 200         & 1        & 13.85        & 5.11      & 2.92        & 6.42  \\
\hdashline
GPT-J+RL  & 6B   & 400         & 1        & 14.61        & 5.44      & 3.65        & 6.92  \\
GPT-J+RL  & 6B   & 800         & 1        & 15.66        & 6.04      & 4.16        & 7.59  \\
GPT-J+RL  & 6B   & 1000        & 1        &   15.87           &   6.16        &   4.24          &    7.72   \\
\hline
CodeT5 & 770M &   100          & 1        &   13.41&	4.29&	2.10&	5.67  \\
CodeT5+RL & 770M &   100          & 1        &  12.63&	4.41&	2.60&	5.69   \\ \hdashline
CodeT5 & 770M &   200          & 1        &  14.65&	4.81&	2.38&	6.29 \\
CodeT5+RL & 770M &   200          & 1     & 14.56&	5.02&	2.94&	6.51  \\ \hdashline
CodeT5+RL & 770M &   400          & 1        & 14.88&	5.68&	3.67&	7.12 \\
CodeT5+RL & 770M &   800          & 1        &16.09&	5.83&	4.30&	7.57 \\
CodeT5+RL & 770M &   1000          & 1        & 16.27&	6.00&	4.27&	7.71  \\
\hline
\end{tabular}
}
\end{table}



\begin{table}[htbp]
\centering
\caption{Results of $5@k$ on APPS:}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lccccccc}
\hline
Model     & Size & Filter from & Attempts & Introductory & Interview & Competition & All   \\
\hline
Codex     & 12B  & 1000        & 5        & 24.52        & 3.23      & 3.08        & 7.46  \\
AlphaCode & 1B   & 1000        & 5        & 14.36        & 5.63      & 4.58        & 7.17  \\
AlphaCode & 1B   & 10000       & 5        & 18.18        & 8.21      & 6.65        & 9.89  \\
AlphaCode & 1B   & 50000       & 5        & 20.36        & 9.66      & 7.75        & 11.42 \\
\hline
GPT-J  & 6B   & 100         & 5        & 19.19	& 6.23	& 3.55	& 8.29 \\
GPT-J+RL  & 6B   & 100         & 5        & 19.49        & 6.06      & 4.64        & 8.46  \\
\hdashline
GPT-J  & 6B   & 200         & 5        &  20.69	 & 7.21	 & 4.44	 & 9.35  \\
GPT-J+RL  & 6B   & 200         & 5        & 21.24        & 7.09      & 5.69        & 9.64  \\
\hdashline
GPT-J+RL  & 6B   & 400         & 5        & 22.24        & 7.88      & 6.40         & 10.46 \\
GPT-J+RL  & 6B   & 800         & 5        & 23.88        & 8.66      & 7.80         & 11.53 \\
GPT-J+RL  & 6B   & 1000        & 5        &   24.11           &    8.89       &    8.09         &  11.77     \\
\hline
CodeT5 & 770M &    100         & 5        &20.24&	5.37&	4.07&	8.08 \\
CodeT5+RL & 770M &    100         & 5        &19.79&	6.07&	4.29&	8.46\\ \hdashline
CodeT5 & 770M &    200         & 5        & 21.85&	6.46&	4.72&	9.19\\
CodeT5+RL & 770M &    200         & 5        &20.41&	6.86&	5.85&	9.37\\ \hdashline
CodeT5+RL & 770M &    400         & 5        & 22.81&	7.86&	6.86&	10.65 \\ 
CodeT5+RL & 770M &    800         & 5        &  24.26&	8.45&	7.80&	11.48  \\ 
CodeT5+RL & 770M &    1000         & 5        &  24.78&	8.75&	8.33&	11.87 \\ 
\hline
\end{tabular}
}
\end{table}



==> tables/n_pass_k_v1.tex <==
\begin{table}[htbp]
\centering
%\caption{Results of $1@k$ on APPS:}
\caption{Results of $1@k$ (in \%) on APPS:
RL denotes our RL finetuning method. NS: nucleus sampling, SS: seed sampling.}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lcccccccc}
\hline
Model     & Size & Sampling & Filter from & Attempts & Introductory & Interview & Competition & All   \\
\hline
Codex     & 12B  &NS & 1000        & 1        & 22.78        & 2.64      & 3.04        & 6.75  \\
\hline
%GPT-J  & 6B   & 100         & 1        &    12.24	& 4.85	& 1.91	& 5.74 \\
%GPT-J+RL  & 6B   & 100         & 1        & 13.08        & 4.93      & 2.26        & 6.03  \\
%\hdashline
GPT-J  & 6B  &NS & 200         & 1        &    13.40	 & 5.35	 & 2.40	 & 6.37 \\
GPT-J+RL  & 6B   &NS & 200         & 1        & 13.85        & 5.11      & 2.92        & 6.42  \\
%\hdashline
%GPT-J+RL  & 6B   & 400         & 1        & 14.61        & 5.44      & 3.65        & 6.92  \\
%GPT-J+RL  & 6B   & 800         & 1        & 15.66        & 6.04      & 4.16        & 7.59  \\
%GPT-J+RL  & 6B   & 1000        & 1        &   15.87           &   6.16        &   4.24          &    7.72   \\
\hline
%CodeT5 & 770M &   100          & 1        &   13.41&	4.29&	2.10&	5.67  \\
%CodeT5+RL & 770M &   100          & 1        &  12.63&	4.41&	2.60&	5.69   \\ \hdashline
CodeT5 & 770M &NS &   200          & 1        &  14.65&	4.81&	2.38&	6.29 \\
CodeT5+RL & 770M &NS &   200          & 1     & 14.56&	5.02&	2.94&	6.51  \\ 
%CodeT5+RL & 770M &SS &   200          & 1     & 16.45&	6.21&	4.33&	7.88  \\ 
\hdashline
%CodeT5+RL & 770M &   400          & 1        & 14.88&	5.68&	3.67&	7.12 \\
%CodeT5+RL & 770M &   400          & 1        & 14.88&	5.68&	3.67&	7.12 \\
%CodeT5+RL & 770M &   800          & 1        &16.09&	5.83&	4.30&	7.57 \\
%\hdashline
CodeT5+RL & 770M &NS &   1000          & 1        & 16.27&	6.00&	4.27&	7.71  \\
CodeT5+RL & 770M &SS &   1000          & 1        & 16.65&	6.23&	4.38&	7.94  \\
\hline
\end{tabular}
}
\end{table}



\begin{table}[htbp]
\centering
\caption{Results of $5@k$ (in \%) on APPS:
RL denotes our RL finetuning method. NS: nucleus sampling, SS: seed sampling.}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lccccccccc}
\hline
Model     & Size & Sampling & Filter from & Attempts & Introductory & Interview & Competition & All   \\
\hline
Codex     & 12B  &NS & 1000        & 5        & 24.52        & 3.23      & 3.08        & 7.46  \\
AlphaCode & 1B   &NS& 1000        & 5        & 14.36        & 5.63      & 4.58        & 7.17  \\
AlphaCode & 1B   &NS& 10000       & 5        & 18.18        & 8.21      & 6.65        & 9.89  \\
AlphaCode & 1B   &NS& 50000       & 5        & 20.36        & 9.66      & 7.75        & 11.42 \\
\hline
%GPT-J  & 6B   & 100         & 5        & 19.19	& 6.23	& 3.55	& 8.29 \\
%GPT-J+RL  & 6B   & 100         & 5        & 19.49        & 6.06      & 4.64        & 8.46  \\
%\hdashline
GPT-J  & 6B   &NS& 200         & 5        &  20.69	 & 7.21	 & 4.44	 & 9.35  \\
GPT-J+RL  & 6B   &NS& 200         & 5        & 21.24        & 7.09      & 5.69        & 9.64  \\
%\hdashline
%GPT-J+RL  & 6B   & 400         & 5        & 22.24        & 7.88      & 6.40         & 10.46 \\
%GPT-J+RL  & 6B   & 800         & 5        & 23.88        & 8.66      & 7.80         & 11.53 \\
%GPT-J+RL  & 6B   & 1000        & 5        &   24.11           &    8.89       &    8.09         &  11.77     \\
\hline
%CodeT5 & 770M &    100         & 5        &20.24&	5.37&	4.07&	8.08 \\
%CodeT5+RL & 770M &    100         & 5        &19.79&	6.07&	4.29&	8.46\\ \hdashline
CodeT5 & 770M &NS&    200         & 5        & 21.85&	6.46&	4.72&	9.19\\
CodeT5+RL & 770M &NS&    200         & 5        &20.41&	6.86&	5.85&	9.37\\ \hdashline
%CodeT5+RL & 770M &SS&    200         & 5        &24.43&	8.47&	7.83&	11.54\\ \hdashline
%CodeT5+RL & 770M &    400         & 5        & 22.81&	7.86&	6.86&	10.65 \\ 
%CodeT5+RL & 770M &    800         & 5        &  24.26&	8.45&	7.80&	11.48  \\ 
CodeT5+RL & 770M &NS&    1000         & 5        &  24.78&	8.75&	8.33&	11.87 \\ 
CodeT5+RL & 770M &SS&    1000         & 5        &  24.43&	8.63&	8.15&	11.69 \\ 
\hline
\end{tabular}
}
\end{table}



==> tables/n_pass_k_v2.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\small
%\caption{Results of $1@k$ on APPS:}
\caption{Results on APPS: ``Intro'': introductory, ``Inter'': interview, ``Comp'': competition-level tasks}
\label{app_tab:n_pass_k}
%\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lcc|cccc|cccc}
\hline
\multicolumn{1}{c}{}                        &                        &                     & \multicolumn{4}{c|}{\emph{1@k}}                                        & \multicolumn{4}{c}{\emph{5@k}}                                         \\
\cline{4-11}
\multicolumn{1}{c}{\multirow{-2}{*}{Model}} & \multirow{-2}{*}{Size} & \multirow{-2}{*}{$k$} & Intro          & Inter         & Comp          & All           & Intro          & Inter         & Comp          & All            \\
\hline
\multicolumn{11}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM}                                                                                                                                                                    \\
\hline
Codex                                       & 12B                    & 1000                & \textbf{22.78} & 2.64          & 3.04          & 6.75          & {24.52}          & 3.23          & 3.08          & 7.46           \\
AlphaCode                                   & 1B                     & 1000                & -              & -             & -             & -             & 14.36          & 5.63          & 4.58          & 7.17           \\
AlphaCode                                   & 1B                     & 10000               & -              & -             & -             & -             & 18.18          & 8.21          & 6.65          & 9.89           \\
AlphaCode                                   & 1B                     & 50000               & -              & -             & -             & -             & 20.36          & \textbf{9.66} & 7.75          & 11.42          \\
GPT-J                                       & 6B                     & 200                 & 13.40          & 5.35          & 2.40          & 6.37          & 20.69          & 7.21          & 4.44          & 9.35           \\
CodeT5                                      & 770M                   & 200                 & 14.65          & 4.81          & 2.38          & 6.29          & 21.85          & 6.46          & 4.72          & 9.19           \\
\hline
\multicolumn{11}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM + CodeRL}                                                                                                                                                           \\
\hline
GPT-J                                       & 6B                     & 200                 & 13.85          & 5.11          & 2.92          & 6.42          & 21.24          & 7.09          & 5.69          & 9.64           \\
CodeT5                                 & 770M                   & 200                 & 14.56          & 5.02          & 2.94          & 6.51          & 20.41          & 6.86          & 5.85          & 9.37           \\
CodeT5                                  & 770M                   & 1000                & 16.27          & 6.00          & \textbf{4.27}          & 7.71          & \textbf{24.78} & 8.75          & \textbf{8.33} & \textbf{11.87} \\
%CodeT5 (CS)                                 & 770M                   & 1000                & 16.65          & \textbf{6.23} & \textbf{4.38} & \textbf{7.94} & 24.43          & 8.63          & 8.15          & 11.69         \\
CodeT5 (CS)                                 & 770M                   & 1000                & 16.52          & \textbf{6.16} & {4.15} & \textbf{7.83} & 24.49          & 8.58          & {7.82}          & {11.61}     \\

\hline
\end{tabular}
%}
\vspace{-0.1in}
\end{table}

==> tables/n_pass_k_v3.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\small
%\caption{Results of $1@k$ on APPS:}
\caption{Results on APPS: ``Intro'': introductory, ``Inter'': interview, ``Comp'': competition-level tasks}
\label{tab:n_pass_k}
\resizebox{0.9\textwidth}{!} {
\begin{tabular}{lcc|cccc|cccc}
\hline
\multicolumn{1}{c}{}                        &                        &                     & \multicolumn{4}{c|}{\emph{1@k}}                                        & \multicolumn{4}{c}{\emph{5@k}}                                         \\
\cline{4-11}
\multicolumn{1}{c}{\multirow{-2}{*}{Model}} & \multirow{-2}{*}{Size} & \multirow{-2}{*}{$k$} & Intro          & Inter         & Comp          & All           & Intro          & Inter         & Comp          & All            \\
\hline
%\multicolumn{11}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM}                                                                                                                                                                    \\\hline
Codex                                       & 12B                    & 1000                & \textbf{22.78} & 2.64          & 3.04          & 6.75          & {24.52}          & 3.23          & 3.08          & 7.46           \\
AlphaCode                                   & 1B                     & 1000                & -              & -             & -             & -             & 14.36          & 5.63          & 4.58          & 7.17           \\
AlphaCode                                   & 1B                     & 10000               & -              & -             & -             & -             & 18.18          & 8.21          & 6.65          & 9.89           \\
AlphaCode                                   & 1B                     & 50000               & -              & -             & -             & -             & 20.36          & \textbf{9.66} & 7.75          & 11.42          \\
%GPT-J                                       & 6B                     & 200                 & 13.40          & 5.35          & 2.40          & 6.37          & 20.69          & 7.21          & 4.44          & 9.35           \\
%CodeT5                                      & 770M                   & 200                 & 14.65          & 4.81          & 2.38          & 6.29          & 21.85          & 6.46          & 4.72          & 9.19           \\
\hline
%\multicolumn{11}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM + CodeRL}                                                                                                                                                           \\\hline
%GPT-J                                       & 6B                     & 200                 & 13.85          & 5.11          & 2.92          & 6.42          & 21.24          & 7.09          & 5.69          & 9.64           \\
%CodeT5                                 & 770M                   & 200                 & 14.56          & 5.02          & 2.94          & 6.51          & 20.41          & 6.86          & 5.85          & 9.37           \\
%CodeT5                                  & 770M                   & 1000                & 16.27          & 6.00          & \textbf{4.27}          & 7.71          & \textbf{24.78} & 8.75          & \textbf{8.33} & \textbf{11.87} \\
%CodeT5 (CS)                                 & 770M                   & 1000                & 16.65          & \textbf{6.23} & \textbf{4.38} & \textbf{7.94} & 24.43          & 8.63          & 8.15          & 11.69         \\
CodeT5+CodeRL                                 & 770M                   & 1000                & 16.52          & \textbf{6.16} & {4.15} & \textbf{7.83} & 24.49          & 8.58          & {7.82}          & {11.61}     \\

\hline
\end{tabular}
}
\vspace{-0.1in}
\end{table}

==> tables/pass_k.tex <==






% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\small
\caption{Results on APPS: ``Intro'': introductory, ``Inter'': interview, ``Comp'': competition-level tasks}
\label{app_tab:pass_k}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lc|cccc|cccc|cccc}
\hline
\multicolumn{1}{c}{}                        &                        & \multicolumn{4}{c|}{\emph{pass@1}}                                       & \multicolumn{4}{c|}{\emph{pass@5}}                                        & \multicolumn{4}{c}{\emph{pass@1000}}                                        \\ 
\cline{3-14}
\multicolumn{1}{c}{\multirow{-2}{*}{Model}} & \multirow{-2}{*}{Size} & Intro         & Inter         & Comp          & All           & Intro          & Inter         & Comp          & All           & Intro          & Inter          & Comp           & All            \\\hline
\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM}                                                                                                                                                                                                                \\ \hline
Codex                                       & 12B                    & 4.14          & 0.14          & 0.02          & 0.92          & 9.65           & 0.51          & 0.09          & 2.25          & 25.02          & 3.70           & 3.23           & 7.87           \\
AlphaCode                                   & 1B                     & -             & -             & -             & -             & -              & -             & -             & -             & 17.67          & 5.24           & 7.06           & 8.09           \\
GPT2                                        & 1.5B                   & 1.30          & 0.70          & 0.00          & 0.68          & 3.60           & 1.03          & 0.00          & 1.34          & -              & -              & -              & -              \\
GPT-Neo                                     & 2.7B                   & 3.90          & 0.57          & 0.00          & 1.12          & 5.50           & 0.80          & 0.00          & 1.58          & -              & -              & -              & -              \\
GPT-J                                       & 6B                     & 5.60          & 1.00          & 0.50          & 1.82          & 9.20           & 1.73          & 1.00          & 3.08          & -              & -              & -              & -              \\
CodeT5                                      & 770M                   & 6.60          & 1.03          & 0.30          & 2.00          & 8.80           & 1.67          & 0.70          & 2.90          & - & - & - &-          \\ \hline
\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM + CodeRL}                                                                                                                                                                                                       \\ \hline
GPT2                                        & 1.5B                   & 2.00          & 0.83          & 0.10          & 0.92          & 3.96           & 1.36          & 0.45          & 1.70          & -              & -              & -              & -              \\
GPT-Neo                                     & 2.7B                   & 4.70          & 0.73          & 0.30          & 1.44          & 6.58           & 1.54          & 0.18          & 2.28          & -              & -              & -              & -              \\
GPT-J                                       & 6B                     & 5.20          & 1.27          & 0.30          & 1.86          & 8.38           & 2.29          & 0.73          & 3.20       &    34.50        &  12.40     &   13.70       & 17.08             \\
%CodeT5 (CS)                                 & 770M                   & \textbf{7.36} & \textbf{1.97} & \textbf{0.81} & \textbf{2.82} & \textbf{16.05} & \textbf{4.81} & \textbf{2.64} & \textbf{6.63} & \textbf{38.50} & \textbf{14.80} & \textbf{17.30} & \textbf{20.04} \\
CodeT5                                 & 770M                   & 6.20           & 1.50           & 0.30           & 2.20           & 9.39           & 1.90           & 0.42          & 3.10           &35.30          & 13.33          & 13.60          & 17.78                  \\
CodeT5 (CS)                                 & 770M                   & \textbf{6.77} & \textbf{1.80} & \textbf{0.69} & \textbf{2.57} & \textbf{15.27} & \textbf{4.48} & \textbf{2.36} & \textbf{6.21} & \textbf{38.10} & \textbf{14.33} & \textbf{15.70} & \textbf{19.36} \\
%CodeT5 (NS)                                 & 770M                   & 3.95          & 0.82          & 0.13          & 1.31          & 9.48           & 2.17          & 0.62          & 3.32          & 35.30          & 13.33          & 13.60          & 17.78           \\
\hline
\end{tabular}
}
\end{table}

==> tables/pass_k_combined_v1.tex <==


\begin{table}[t]
\centering
\caption{Results on APPS: ``Intro'': introductory, ``Inter'': interview, ``Comp'': competition-level tasks}
\begin{subtable}[htbp]{1.0\textwidth}
\centering
%\small
\caption{Performance by \emph{pass@k} with $k=\{1,5,1000\}$}
\label{tab:pass_k}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lc|cccc|cccc|cccc}
\hline
\multicolumn{1}{c}{}                        &                        & \multicolumn{4}{c|}{\emph{pass@1}}                                       & \multicolumn{4}{c|}{\emph{pass@5}}                                        & \multicolumn{4}{c}{\emph{pass@1000}}                                        \\ 
\cline{3-14}
\multicolumn{1}{c}{\multirow{-2}{*}{Model}} & \multirow{-2}{*}{Size} & Intro         & Inter         & Comp          & All           & Intro          & Inter         & Comp          & All           & Intro          & Inter          & Comp           & All            \\\hline
%\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM}                                                                                                                                                                                                                \\ \hline
Codex                                       & 12B                    & 4.14          & 0.14          & 0.02          & 0.92          & 9.65           & 0.51          & 0.09          & 2.25          & 25.02          & 3.70           & 3.23           & 7.87           \\
AlphaCode                                   & 1B                     & -             & -             & -             & -             & -              & -             & -             & -             & 17.67          & 5.24           & 7.06           & 8.09           \\
GPT3                                        & 175B                   & 0.20          & 0.03          & 0.00          & 0.06          & -           & -          & -          & -          & -              & -              & -              & -              \\

GPT2                                        & 0.1B                   & 1.00          & 0.33          & 0.00          & 0.40          & 2.70           & 0.73          & 0.00          & 1.02          & -              & -              & -              & -              \\
GPT2                                        & 1.5B                   & 1.30          & 0.70          & 0.00          & 0.68          & 3.60           & 1.03          & 0.00          & 1.34          & -              & -              & -              & -              \\
GPT-Neo                                     & 2.7B                   & 3.90          & 0.57          & 0.00          & 1.12          & 5.50           & 0.80          & 0.00          & 1.58          & -              & -              & -              & -              \\
GPT-J                                       & 6B                     & 5.60          & 1.00          & 0.50          & 1.82          & 9.20           & 1.73          & 1.00          & 3.08          & -              & -              & -              & -              \\
 \hline
%CodeT5                                      & 770M                   & 6.60          & 1.03          & 0.30          & 2.00          & 8.80           & 1.67          & 0.70          & 2.90          & - & - & - &-          \\
%\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM + CodeRL}                                                                                                                                                                                                       \\ \hline
%GPT2                                        & 1.5B                   & 2.00          & 0.83          & 0.10          & 0.92          & 3.96           & 1.36          & 0.45          & 1.70          & -              & -              & -              & -              \\
%GPT-Neo                                     & 2.7B                   & 4.70          & 0.73          & 0.30          & 1.44          & 6.58           & 1.54          & 0.18          & 2.28          & -              & -              & -              & -              \\
%GPT-J                                       & 6B                     & 5.20          & 1.27          & 0.30          & 1.86          & 8.38           & 2.29          & 0.73          & 3.20       &    34.50        &  12.40     &   13.70       & 17.08             \\
%CodeT5 (CS)                                 & 770M                   & \textbf{7.36} & \textbf{1.97} & \textbf{0.81} & \textbf{2.82} & \textbf{16.05} & \textbf{4.81} & \textbf{2.64} & \textbf{6.63} & \textbf{38.50} & \textbf{14.80} & \textbf{17.30} & \textbf{20.04} \\
%CodeT5                                 & 770M                   & 6.20           & 1.50           & 0.30           & 2.20           & 9.39           & 1.90           & 0.42          & 3.10           &35.30          & 13.33          & 13.60          & 17.78                  \\
CodeRL+CodeT5                                 & 770M                   & \textbf{6.77} & \textbf{1.80} & \textbf{0.69} & \textbf{2.57} & \textbf{15.27} & \textbf{4.48} & \textbf{2.36} & \textbf{6.21} & \textbf{38.10} & \textbf{14.33} & \textbf{15.70} & \textbf{19.36} \\
\hdashline
+CodeFixing (k=1)                                 & 770M                   & 6.88 &	1.81 &	0.70	& 2.58	& 15.28	& 4.50	& 2.48	& 6.24	& 38.10	& 14.45	& 15.70	& 19.41 \\
+CodeFixing (k=2)                                 & 770M                   & 7.01	& 2.01	& 0.72	& 2.63	& 16.01	& 5.11	& 2.63	& 6.80	& 39.10	& 16.55	& 16.42	& 20.04 \\
+CodeFixing (k=3)                                 & 770M                   & 7.00	& 1.90&	0.64&	2.60&	15.83&	5.01&	2.55&	6.26&	40.00&	16.01&	16.01&	19.62 \\
+CodeFixing (k=4)                                 & 770M                   & 6.42&	1.94&	0.61&	2.55&	15.88&	5.04&	2.49&	6.30&	39.11&	15.42	&15.90&	19.55 \\
+CodeFixing (random)                                 & 770M                   & 6.77&	1.80&	0.70&	2.57&	15.27&	4.50&	2.36&	6.22&	38.10&	14.40&	15.70	&19.38\\

\hline
\end{tabular}
}
\end{subtable}
\vspace{+0.2in}


\begin{subtable}[htbp]{1.0\textwidth}
\centering
%\small
%\caption{Results of $1@k$ on APPS:}
\caption{Performance by \emph{n@k} with $k$ up to 50000 and $n=\{1,5\}$}
\label{tab:n_pass_k}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lcc|cccc|cccc}
\hline
\multicolumn{1}{c}{}                        &                        &                     & \multicolumn{4}{c|}{\emph{1@k}}                                        & \multicolumn{4}{c}{\emph{5@k}}                                         \\
\cline{4-11}
\multicolumn{1}{c}{\multirow{-2}{*}{Model}} & \multirow{-2}{*}{Size} & \multirow{-2}{*}{$k$} & Intro          & Inter         & Comp          & All           & Intro          & Inter         & Comp          & All            \\
\hline
%\multicolumn{11}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM}                                                                                                                                                                    \\\hline
Codex                                       & 12B                    & 1000                & \textbf{22.78} & 2.64          & 3.04          & 6.75          & \textbf{24.52}          & 3.23          & 3.08          & 7.46           \\
AlphaCode                                   & 1B                     & 1000                & -              & -             & -             & -             & 14.36          & 5.63          & 4.58          & 7.17           \\
AlphaCode                                   & 1B                     & 10000               & -              & -             & -             & -             & 18.18          & 8.21          & 6.65          & 9.89           \\
AlphaCode                                   & 1B                     & 50000               & -              & -             & -             & -             & 20.36          & \textbf{9.66} & 7.75          & 11.42          \\
%GPT-J                                       & 6B                     & 200                 & 13.40          & 5.35          & 2.40          & 6.37          & 20.69          & 7.21          & 4.44          & 9.35           \\
%CodeT5                                      & 770M                   & 200                 & 14.65          & 4.81          & 2.38          & 6.29          & 21.85          & 6.46          & 4.72          & 9.19           \\
\hline
%\multicolumn{11}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM + CodeRL}                                                                                                                                                           \\\hline
%GPT-J                                       & 6B                     & 200                 & 13.85          & 5.11          & 2.92          & 6.42          & 21.24          & 7.09          & 5.69          & 9.64           \\
%CodeT5                                 & 770M                   & 200                 & 14.56          & 5.02          & 2.94          & 6.51          & 20.41          & 6.86          & 5.85          & 9.37           \\
%CodeT5                                  & 770M                   & 1000                & 16.27          & 6.00          & \textbf{4.27}          & 7.71          & \textbf{24.78} & 8.75          & \textbf{8.33} & \textbf{11.87} \\
%CodeT5 (CS)                                 & 770M                   & 1000                & 16.65          & \textbf{6.23} & \textbf{4.38} & \textbf{7.94} & 24.43          & 8.63          & 8.15          & 11.69         \\
CodeRL+CodeT5                                 & 770M                   & 1000                & 16.52          & \textbf{6.16} & \textbf{4.15} & \textbf{7.83} & 24.49          & 8.58          & \textbf{7.82}          & \textbf{11.61}     \\

\hline
\end{tabular}
}
%\vspace{-0.2in}
\end{subtable}
\end{table}

==> tables/pass_k_large.tex <==
\begin{table}[htbp]
\centering
\caption{Results of pass@$k$ with with large $k$ up to 1000 samples on APPS:}
\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{c}{Model} & Size & Attempts & Introductory & Interview & Competition & All   \\\hline
Codex                     & 12B  & 1000     & 25.02        & 3.70      & 3.23        & 7.87  \\
AlphaCode                 & 1B   & 1000     & 17.67        & 5.24      & 7.06        & 8.09  \\
GPT-Neo                   & 2.7B & 100      & 19.10        & 5.30      & 3.70        & 7.74  \\\hline
GPT-J                     & 6B   & 100      & 23.10        & 7.43      & 4.50        & 9.98  \\
GPT-J+RL                  & 6B   & 100      & 23.20        & 7.67      & 5.60        & 10.36 \\
\hdashline
GPT-J                     & 6B   & 200      & 26.00        & 9.10      & 6.70        & 12.00 \\
GPT-J+RL                  & 6B   & 200      & 27.10        & 9.03      & 7.50        & 12.34 \\
\hdashline
GPT-J+RL                  & 6B   & 400      & 30.20        & 10.17      & 10.80        & 14.30 \\
GPT-J+RL                  & 6B   & 800      &  33.80       &  11.73     &   12.80      &  16.36 \\
GPT-J+RL                  & 6B   & 1000      & 34.50        &  12.40     &   13.70       & 17.08  \\\hline

CodeT5                    & 770M & 100      & 24.29 &	6.50 &	4.84 &	9.72 \\
CodeT5+RL                 & 770M & 100      &  22.99 &	7.09 &	5.41 &	9.93 \\ \hdashline
CodeT5                    & 770M & 200      & 27.70 &	8.03 &	6.70 &	11.70 \\
CodeT5+RL                 & 770M & 200      & 26.79 &	8.73 &	7.60 &	12.12  \\  \hdashline
CodeT5+RL                 & 770M & 400      & 30.55 &	10.61&	10.09&	14.50   \\
CodeT5+RL                 & 770M & 800      & 34.18 &	12.66&	12.74&	16.98   \\
CodeT5+RL                 & 770M & 1000     & 35.30 &	13.33&	13.60&	17.78  \\
\hline
\end{tabular}
\end{table}


==> tables/pass_k_large_v1.tex <==
\begin{table}[htbp]
\centering
\caption{Results of pass@$k$ (in \%) with with large $k$ up to 1000 samples on APPS:
RL denotes our RL finetuning method. NS: nucleus sampling, SS: seed sampling.}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lccccccc}
\hline
\multicolumn{1}{c}{Model} & Size & Sampling & Attempts & Introductory & Interview & Competition & All   \\\hline
Codex                     & 12B  &NS & 1000     & 25.02        & 3.70      & 3.23        & 7.87  \\
AlphaCode                 & 1B   &NS & 1000     & 17.67        & 5.24      & 7.06        & 8.09  \\
GPT-Neo                   & 2.7B &NS & 100      & 19.10        & 5.30      & 3.70        & 7.74  \\\hline
%GPT-J                     & 6B   & 100      & 23.10        & 7.43      & 4.50        & 9.98  \\
%GPT-J+RL                  & 6B   & 100      & 23.20        & 7.67      & 5.60        & 10.36 \\
%\hdashline
GPT-J                     & 6B   &NS & 200      & 26.00        & 9.10      & 6.70        & 12.00 \\
GPT-J+RL                  & 6B   &NS & 200      & 27.10        & 9.03      & 7.50        & 12.34 \\
\hline
%\hdashline
%GPT-J+RL                  & 6B   & 400      & 30.20        & 10.17      & 10.80        & 14.30 \\
%GPT-J+RL                  & 6B   & 800      &  33.80       &  11.73     &   12.80      &  16.36 \\
%GPT-J+RL                  & 6B   & 1000      & 34.50        &  12.40     &   13.70       & 17.08  \\\hline

%CodeT5                    & 770M & 100      & 24.29 &	6.50 &	4.84 &	9.72 \\
%CodeT5+RL                 & 770M & 100      &  22.99 &	7.09 &	5.41 &	9.93 \\ \hdashline
CodeT5                    & 770M &NS & 200      & 27.70 &	8.03 &	6.70 &	11.70 \\
CodeT5+RL                 & 770M &NS & 200      & 26.79 &	8.73 &	7.60 &	12.12  \\ 
%CodeT5+RL                 & 770M &SS & 200      & 33.68 &	12.37&	13.82&	16.92  \\  \hdashline
CodeT5+RL                 & 770M &SS & 200      & 29.00 &	9.80&	10.00&	13.68  \\  \hdashline
%CodeT5+RL                 & 770M &NS & 400      & 30.55 &	10.61&	10.09&	14.50   \\
%CodeT5+RL                 & 770M &SS & 400      &35.65 &	13.38&	15.33&	18.23   \\
%\hdashline
%CodeT5+RL                 & 770M &NS & 800      & 34.18 &	12.66&	12.74&	16.98   \\
%CodeT5+RL                 & 770M &SS & 800      & 37.78 &	14.44&	16.81&	19.58   \\
%\hdashline
CodeT5+RL                 & 770M &NS & 1000     & 35.30 &	13.33&	13.60&	17.78  \\
CodeT5+RL                 & 770M &SS & 1000     & 38.50 &	14.80&	17.30&	20.04   \\
\hline
\end{tabular}
}
\end{table}


==> tables/pass_k_small.tex <==
\begin{table}[htbp]
\centering
\caption{Results of pass@1 (in \%) on APPS:}
\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{c}{Model} & Size & Attempts & Introductory & Interview & Competition & All  \\
\hline
Codex                     & 12B  & 1        & 4.14         & 0.14      & 0.02        & 0.92 \\\hline
GPT2                      & 1.5B & 1        & 1.30         & 0.70      & 0.00        & 0.68 \\
GPT2+RL                   & 1.5B & 1        & 2.00         & 0.83      & 0.10        & 0.92 \\\hline
GPT-Neo                   & 2.7B & 1        & 3.90         & 0.57      & 0.00        & 1.12 \\
GPT-Neo+RL                & 2.7B & 1        & 4.70         & 0.73      & 0.30        & 1.44 \\\hline
GPT-J                     & 6B   & 1        & 5.60         & 1.00      & 0.50        & 1.82 \\
GPT-J+RL                  & 6B   & 1        & 5.20         & 1.27      & 0.30        & 1.86 \\\hline
CodeT5                    & 770M & 1        & 6.60         & 1.03      & 0.30        & 2.00 \\
CodeT5+RL                 & 770M & 1        & 6.20         & 1.50      & 0.30      &  2.20\\
\hline 
\end{tabular}
\end{table}


\begin{table}[htbp]
\centering
\caption{Results of pass@5 (in \%) on APPS:}
\begin{tabular}{lcccccc}
\hline
Model      & \multicolumn{1}{l}{Size} & \multicolumn{1}{l}{Attempts} & \multicolumn{1}{l}{Introductory} & \multicolumn{1}{l}{Interview} & \multicolumn{1}{l}{Competition} & \multicolumn{1}{l}{All} \\\hline
Codex      & 12B                      & 5                            & 9.65                             & 0.51                          & 0.09                            & 2.25                    \\\hline
GPT2       & 1.5B                     & 5                            & 3.60                             & 1.03                          & 0.00                            & 1.34                    \\
GPT2+RL    & 1.5B                     & 5                            & 3.96                             & 1.36                          & 0.45                            & 1.70                    \\\hline
GPT-Neo    & 2.7B                     & 5                            & 5.50                             & 0.80                          & 0.00                            & 1.58                    \\
GPT-Neo+RL & 2.7B                     & 5                            & 6.58                             & 1.54                          & 0.18                            & 2.28                    \\\hline
GPT-J      & 6B                       & 5                            & 9.20                             & 1.73                          & 1.00                            & 3.08                    \\
GPT-J+RL   & 6B                       & 5                            & 8.38                             & 2.29                          & 0.73                            & 3.20                     \\\hline
CodeT5     & 770M                     & 5                            & 8.80                             & 1.67                          & 0.70                            & 2.90                    \\
CodeT5+RL  & 770M                     & 5                            & 9.39                             & 1.90                          & 0.42                            & 3.10         \\
\hline
\end{tabular}
\end{table}

==> tables/pass_k_small_v1.tex <==
\begin{table}[htbp]
\centering
\caption{Results of pass@1 (in \%) on APPS:
RL denotes our RL finetuning method. NS: nucleus sampling, BS: beam search, SS: seed sampling.}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lccccccc}
\hline
\multicolumn{1}{c}{Model} & Size & Sampling & Attempts & Introductory & Interview & Competition & All  \\
\hline
Codex                     & 12B  &NS & 1        & 4.14         & 0.14      & 0.02        & 0.92 \\\hline
GPT2                      & 1.5B & BS & 1        & 1.30         & 0.70      & 0.00        & 0.68 \\
GPT2+RL                   & 1.5B &BS & 1        & 2.00         & 0.83      & 0.10        & 0.92 \\\hline
GPT-Neo                   & 2.7B &BS& 1        & 3.90         & 0.57      & 0.00        & 1.12 \\
GPT-Neo+RL                & 2.7B &BS& 1        & 4.70         & 0.73      & 0.30        & 1.44 \\\hline
GPT-J                     & 6B   &BS& 1        & 5.60         & 1.00      & 0.50        & 1.82 \\
GPT-J+RL                  & 6B   &BS& 1        & 5.20         & 1.27      & 0.30        & 1.86 \\\hline
CodeT5                    & 770M &BS& 1        & 6.60         & 1.03      & 0.30        & 2.00 \\
CodeT5+RL                 & 770M &BS& 1        & 6.20         & 1.50      & 0.30      &  2.20\\
\hdashline
CodeT5+RL                 & 770M &NS& 1        &3.95 &	0.82 &	0.13 &	1.31    \\
%CodeT5+RL                  & 770M &SS &  1        & 7.57 &	2.03 &	0.88 &	2.91 \\
CodeT5+RL                  & 770M &SS &  1        & 7.36 &	1.97 &	0.81 &	2.82 \\
\hline 
\end{tabular}
}
\end{table}


\begin{table}[htbp]
\centering
\caption{Results of pass@5 (in \%) on APPS:
RL denotes our RL finetuning method. NS: nucleus sampling, BS: beam search, SS: seed sampling.}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lccccccc}
\hline
Model      & \multicolumn{1}{l}{Size} & \multicolumn{1}{l}{Sampling} & \multicolumn{1}{l}{Attempts} & \multicolumn{1}{l}{Introductory} & \multicolumn{1}{l}{Interview} & \multicolumn{1}{l}{Competition} & \multicolumn{1}{l}{All} \\\hline
Codex      & 12B             &NS          & 5                            & 9.65                             & 0.51                          & 0.09                            & 2.25                    \\\hline
GPT2       & 1.5B      &BS               & 5                            & 3.60                             & 1.03                          & 0.00                            & 1.34                    \\
GPT2+RL    & 1.5B     &BS                & 5                            & 3.96                             & 1.36                          & 0.45                            & 1.70                    \\\hline
GPT-Neo    & 2.7B     &BS                & 5                            & 5.50                             & 0.80                          & 0.00                            & 1.58                    \\
GPT-Neo+RL & 2.7B    &BS                 & 5                            & 6.58                             & 1.54                          & 0.18                            & 2.28                    \\\hline
GPT-J      & 6B    &BS                   & 5                            & 9.20                             & 1.73                          & 1.00                            & 3.08                    \\
GPT-J+RL   & 6B    &BS                   & 5                            & 8.38                             & 2.29                          & 0.73                            & 3.20                     \\\hline
CodeT5     & 770M      &BS               & 5                            & 8.80                             & 1.67                          & 0.70                            & 2.90                    \\
CodeT5+RL  & 770M   &BS                  & 5                            & 9.39                             & 1.90                          & 0.42                            & 3.10         \\
\hdashline
CodeT5+RL  & 770M   &NS                  & 5                            & 9.48 & 2.17 &	0.62 &	3.32        \\
%CodeT5+RL  & 770M   &SS                  & 5                            & 17.05 &	5.22 &	3.14 &	7.17        \\
CodeT5+RL  & 770M   &SS                  & 5                            & 16.05 &	4.81 &	2.64 &	6.63        \\
\hline
\end{tabular}
}
\end{table}

==> tables/pass_k_small_v2.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[htbp]
\centering
\small
\caption{Results of pass@1 (in \%) on APPS:
RL denotes our RL finetuning method. NS: nucleus sampling, BS: beam search, SS: seed sampling.}
%\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lccccccccc}
\multicolumn{1}{c}{}                        &                        & \multicolumn{4}{c}{Pass@1}                                    & \multicolumn{4}{c}{Pass@5}                                     \\
\multicolumn{1}{c}{\multirow{-2}{*}{Model}} & \multirow{-2}{*}{Size} & Intro         & Inter         & Comp          & All           & Intro          & Inter         & Comp          & All           \\
\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}Pretrained LM}                                                                                                                                            \\
Codex                                       & 12B                    & 4.14          & 0.14          & 0.02          & 0.92          & 9.65           & 0.51          & 0.09          & 2.25          \\
GPT2                                        & 1.5B                   & 1.30          & 0.70          & 0.00          & 0.68          & 3.60           & 1.03          & 0.00          & 1.34          \\
GPT-Neo                                     & 2.7B                   & 3.90          & 0.57          & 0.00          & 1.12          & 5.50           & 0.80          & 0.00          & 1.58          \\
GPT-J                                       & 6B                     & 5.60          & 1.00          & 0.50          & 1.82          & 9.20           & 1.73          & 1.00          & 3.08          \\
CodeT5                                      & 770M                   & 6.60          & 1.03          & 0.30          & 2.00          & 8.80           & 1.67          & 0.70          & 2.90          \\
\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}Pretrained LM + CodeRL}                                                                                                                                   \\
GPT2                                        & 1.5B                   & 2.00          & 0.83          & 0.10          & 0.92          & 3.96           & 1.36          & 0.45          & 1.70          \\
GPT-Neo                                     & 2.7B                   & 4.70          & 0.73          & 0.30          & 1.44          & 6.58           & 1.54          & 0.18          & 2.28          \\
GPT-J                                       & 6B                     & 5.20          & 1.27          & 0.30          & 1.86          & 8.38           & 2.29          & 0.73          & 3.20          \\
CodeT5                                      & 770M                   & \textbf{7.36} & \textbf{1.97} & \textbf{0.81} & \textbf{2.82} & \textbf{16.05} & \textbf{4.81} & \textbf{2.64} & \textbf{6.63}
\end{tabular}
%}
\end{table}

==> tables/pass_k_v1.tex <==






% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\small
\caption{Results on APPS: ``Intro'': introductory, ``Inter'': interview, ``Comp'': competition-level tasks}
\label{tab:pass_k}
\resizebox{1.0\textwidth}{!} {
\begin{tabular}{lc|cccc|cccc|cccc}
\hline
\multicolumn{1}{c}{}                        &                        & \multicolumn{4}{c|}{\emph{pass@1}}                                       & \multicolumn{4}{c|}{\emph{pass@5}}                                        & \multicolumn{4}{c}{\emph{pass@1000}}                                        \\ 
\cline{3-14}
\multicolumn{1}{c}{\multirow{-2}{*}{Model}} & \multirow{-2}{*}{Size} & Intro         & Inter         & Comp          & All           & Intro          & Inter         & Comp          & All           & Intro          & Inter          & Comp           & All            \\\hline
%\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM}                                                                                                                                                                                                                \\ \hline
Codex                                       & 12B                    & 4.14          & 0.14          & 0.02          & 0.92          & 9.65           & 0.51          & 0.09          & 2.25          & 25.02          & 3.70           & 3.23           & 7.87           \\
AlphaCode                                   & 1B                     & -             & -             & -             & -             & -              & -             & -             & -             & 17.67          & 5.24           & 7.06           & 8.09           \\
GPT2                                        & 1.5B                   & 1.30          & 0.70          & 0.00          & 0.68          & 3.60           & 1.03          & 0.00          & 1.34          & -              & -              & -              & -              \\
GPT-Neo                                     & 2.7B                   & 3.90          & 0.57          & 0.00          & 1.12          & 5.50           & 0.80          & 0.00          & 1.58          & -              & -              & -              & -              \\
GPT-J                                       & 6B                     & 5.60          & 1.00          & 0.50          & 1.82          & 9.20           & 1.73          & 1.00          & 3.08          & -              & -              & -              & -              \\
CodeT5                                      & 770M                   & 6.60          & 1.03          & 0.30          & 2.00          & 8.80           & 1.67          & 0.70          & 2.90          & - & - & - &-          \\ \hline
%\multicolumn{14}{c}{\cellcolor[HTML]{EFEFEF}Pretrained LM + CodeRL}                                                                                                                                                                                                       \\ \hline
%GPT2                                        & 1.5B                   & 2.00          & 0.83          & 0.10          & 0.92          & 3.96           & 1.36          & 0.45          & 1.70          & -              & -              & -              & -              \\
%GPT-Neo                                     & 2.7B                   & 4.70          & 0.73          & 0.30          & 1.44          & 6.58           & 1.54          & 0.18          & 2.28          & -              & -              & -              & -              \\
%GPT-J                                       & 6B                     & 5.20          & 1.27          & 0.30          & 1.86          & 8.38           & 2.29          & 0.73          & 3.20       &    34.50        &  12.40     &   13.70       & 17.08             \\
%CodeT5 (CS)                                 & 770M                   & \textbf{7.36} & \textbf{1.97} & \textbf{0.81} & \textbf{2.82} & \textbf{16.05} & \textbf{4.81} & \textbf{2.64} & \textbf{6.63} & \textbf{38.50} & \textbf{14.80} & \textbf{17.30} & \textbf{20.04} \\
%CodeT5                                 & 770M                   & 6.20           & 1.50           & 0.30           & 2.20           & 9.39           & 1.90           & 0.42          & 3.10           &35.30          & 13.33          & 13.60          & 17.78                  \\
CodeT5+CodeRL                                 & 770M                   & \textbf{6.77} & \textbf{1.80} & \textbf{0.69} & \textbf{2.57} & \textbf{15.27} & \textbf{4.48} & \textbf{2.36} & \textbf{6.21} & \textbf{38.10} & \textbf{14.33} & \textbf{15.70} & \textbf{19.36} \\
%CodeT5 (NS)                                 & 770M                   & 3.95          & 0.82          & 0.13          & 1.31          & 9.48           & 2.17          & 0.62          & 3.32          & 35.30          & 13.33          & 13.60          & 17.78           \\
\hline
\end{tabular}
}
\end{table}
